Towards a Value-Complemented Framework for Enabling Human Monitoring in Cyber-Physical Systems

[Context and Motivation]: Cyber-Physical Systems (CPS) have become relevant in a wide variety of different domains, integrating hardware and software, often operating in an emerging and uncertain environment where human actors actively or passively engage with the CPS. To ensure correct and safe operation, and self-adaptation, monitors are used for collecting and analyzing diverse runtime information. [Problem]: However, monitoring humans at runtime, collecting potentially sensitive information about their actions and behavior, comes with significant ramifications that can severely hamper the successful integration of human-machine collaboration. Requirements engineering (RE) activities must integrate diverse human values, including Privacy, Security, and Self-Direction during system design, to avoid involuntary data sharing or misuse. [Principal Ideas]: In this research preview, we focus on the importance of incorporating these aspects in the RE lifecycle of eliciting and creating runtime monitors. [Contribution]: We derived an initial conceptual framework, building on the value taxonomy introduced by Schwartz and human value integrated Software Engineering by Whittle, further leveraging the concept of value tactics. The goal is to tie functional and non-functional monitoring requirements to human values and establish traceability between values, requirements, and actors. Based on this, we lay out a research roadmap guiding our ongoing work in this area.

==> scikgtex.tex <==
% Metainformation
\metatitle*{Towards a Value-Complemented Framework for Enabling Human Monitoring in Cyber-Physical Systems}
\metaauthor*{Zoe Pfister}
\metaauthor*{Michael Vierhauser}
\metaauthor*{Rebekka Wohlrab}
\metaauthor*{Ruth Breu}
\researchfield*{value-based requirements engineering}
\researchfield*{requirements engineering}
\researchfield*{human values in requirements engineering}
% 
\contribution*[2]{supplementary material repository}{https://github.com/Ethical-Human-Machine-Interaction/vcmf}
